Snowmass 2021 White Paper: The Selena Neutrino Experiment

Imaging devices made from an ionization target layer of amorphous selenium (aSe) coupled to a silicon complementary metal-oxide-semiconductor (CMOS) active pixel array for charge readout are a promising technology for neutrino physics. The high spatial resolution in a solid-state target provides unparalleled rejection of backgrounds from natural radioactivity in the search for neutrinoless $\beta\beta$ decay and for electron neutrino ($\nu_e$) spectroscopy with $^{82}$Se. In this white paper, we summarize the broad scientific program of a large imaging detector with a 10-ton target of $^{82}$Se. We review the detector technology, and outline the ongoing research program to realize this experiment.

==> Selena White Paper/header.tex <==
\usepackage[T1]{fontenc} 
\usepackage{amsmath}    % need for subequations
\usepackage{graphicx}   % need for figures
\usepackage{verbatim}   % useful for program listings
\usepackage{color}      % use if color is used in text
%\usepackage{subfigure}  % use for side-by-side figures
\usepackage[caption=false]{subfig}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage[%
hidelinks,
  breaklinks=true,%
  colorlinks=true,%
  linkcolor=blue,anchorcolor=blue,%
  citecolor=blue,filecolor=blue,%
  menucolor=blue,%
  urlcolor=blue]{hyperref}  % use for hypertext links, including those to external documents and URLs
\usepackage[separate-uncertainty,retain-explicit-plus,per-mode=symbol,binary-units]{siunitx}
\usepackage{rotate}
\usepackage{rotating}
\usepackage{bm}
\usepackage{paralist}
\usepackage{wrapfig}
\usepackage{caption3}
\usepackage{longtable}
\usepackage{appendix}
\usepackage{vruler}
\usepackage{enumitem}
\usepackage[version=4]{mhchem}
%\linespread{1.0}
\linespread{0.901} 
\usepackage{chemarrow}

%\renewcommand{\thefigure}{\arabic{chapter}.\arabic{figure}}

\newenvironment{compactlist}{
 \begin{list}{{$\bullet$}}{
  \setlength\partopsep{2pt}
  \setlength\parskip{2pt}
  \setlength\parsep{2pt}
  \setlength\topsep{2pt}
  \setlength\itemsep{2pt}
  \setlength{\itemindent}{2pt}
  %\setlength{\itemindent}{\leftmargin}
  %\setlength{\leftmargin}{0pt}
  \setlength{\leftmargin}{12pt}
 }
}{
 \end{list}
}

\renewcommand{\theparagraph}{\arabic{paragraph}}

\usepackage{titlesec}
\titleformat{\section}{\normalfont\fontsize{11}{15}\bfseries\centering}{\thesection.}{1em}{\uppercase}
%\titleformat{\subsection}{\normalfont\fontsize{11}{15}\bfseries\centering}{\thesubsection.}{1em}{}
\titleformat{\subsection}{\normalfont\fontsize{11}{15}\bfseries\centering}{\thesection\,\thesubsection.}{1em}{}
% UNCOMMENT BELOW IF YOU WANT TO LOSE LESS SPACE IN TITLES AND WHITE SPACE AROUND THEM
%\usepackage{titlesec}
\titlespacing{\section}{0pt}{0.8\baselineskip}{0.5\baselineskip}
\titlespacing{\subsection}{0pt}{0.8\baselineskip}{0.5\baselineskip}
\titlespacing{\subsubsection}{0pt}{0.4\baselineskip}{0.2\baselineskip}
%\titlespacing{\paragraph}{0pt}{0.4\baselineskip}{0.2\baselineskip}

\renewcommand{\thetable}{\arabic{table}}
\renewcommand{\thefigure}{\arabic{figure}}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\Alph{subsection}}
%\renewcommand{\thesubfigure}{\arabic{subfigure}}

\renewcommand{\bibsection}{\center{\normalsize{\bf REFERENCES}}}
\renewcommand{\bibfont}{\normalsize}

%\usepackage[colorlinks=true,pdfstartview=FitV,linkcolor=blue,citecolor=blue, urlcolor=blue]{hyperref}
%---
\setlength\textwidth{6.45in}
\setlength\textheight{8.95in}
\setlength\oddsidemargin{0in}
\setlength\evensidemargin{0in}
\setlength\topmargin{-0.075in}
\setlength\headheight{0in}
\setlength\headsep{0.1in}
%---
\setlength\textfloatsep{2pt}
\setlength\abovecaptionskip{4pt}
%\setlength{\skip\footins}{10pt}
%---
%\renewcommand{\familydefault}{\sfdefault}
%---
\newcommand{\myref}[1]{\href{http://#1}{http://#1}}
%---
\newcommand{\up}[1]{$^{#1}$}
\newcommand{\down}[1]{$_{#1}$}
\newcommand{\cso}[1]{\mbox{10$^{-#1}$\,cm$^2$}}
\newcommand{\cst}[2]{\mbox{#2$\times$10$^{-#1}$\,cm$^2$}}
\newcommand{\omag}[1]{\mbox{$\mathcal{O}(\mbox{#1})$}}
\newcommand{\iso}[2]{\ensuremath{^{#2}\mathrm{#1}}}
\newcommand{\powero}[1]{\mbox{10$^{#1}$}}
\newcommand{\powert}[2]{\mbox{#2$\times$10$^{#1}$}}
\newcommand{\ev}{\mbox{eV\,$c^{-2}$}}
\newcommand{\eve}{\mbox{eV$_{\rm ee}$}}
\newcommand{\evr}{\mbox{eV$_{\rm nr}$}}
\newcommand{\um}{\mbox{$\mu$m}}
\newcommand{\us}{\mbox{$\mu$s}}
\newcommand{\dru}{\mbox{keV$^{-1}$\,kg$^{-1}$\,d$^{-1}$}}
%\newcommand{\dru}{\mbox{keV$_{\rm ee}^{-1}$\,kg$^{-1}$\,d$^{-1}$}}
\newcommand{\kgd}{\mbox{kg$^{-1}$\,d$^{-1}$}}
\newcommand{\cmd}{\mbox{cm$^{-2}$\,d$^{-1}$}}
\newcommand{\lcu}{\mbox{$e^-$\,pix$^{-1}$\,d$^{-1}$}}
%---
\newcommand{\sxy}{\mbox{$\sigma_{xy}$}}
\newcommand{\hlife}{\mbox{$\tau_{1/2}$}}
%---
\newcommand{\bb}{\mbox{$\beta\beta$}}
\newcommand{\bbonu}{\mbox{$\beta\beta0\nu$}}
\newcommand{\bbznu}{\mbox{$\beta\beta0\nu$}}
\newcommand{\mbb}{\mbox{$m_{\beta\beta}$}}
\newcommand{\Qbb}{\mbox{$Q_{\beta\beta}$}}
\newcommand{\bbzn}{\mbox{$0\nu\beta\beta$}}
\newcommand{\bbtn}{\mbox{$2\nu\beta\beta$}}
\newcommand{\tozn}{\mbox{$\tau^{0\nu}_{1/2}$}}
\newcommand{\totn}{\mbox{$\tau^{2\nu}_{1/2}$}}
\newcommand{\mlight}{\mbox{$m_{\mbox{\tiny{lightest}}}$}}
\newcommand{\gr}{\mbox{$\gamma$-ray}}
\newcommand{\nue}{\mbox{$\nu_e$}}
\newcommand{\ise}{\mbox{$^{82}$Se}}
%---
\newcommand{\trit}{\ce{^{3}H}}
\newcommand{\sitwo}{\ce{^{32}Si}}
\newcommand{\ptwo}{\ce{^{32}P}}
\newcommand{\pbten}{\ce{^{210}Pb}}
\newcommand{\poten}{\ce{^{210}Po}}
\newcommand{\biten}{\ce{^{210}Bi}}
\newcommand{\ura}{\ce{^{238}U}}
\newcommand{\tho}{\ce{^{232}Th}}
\newcommand{\kfo}{\ce{^{40}K}}
\newcommand{\sbfo}{\ce{^{124}Sb}}
\newcommand{\ben}{\ce{^{9}Be}}
\newcommand{\cosev}{\ce{^{57}Co}}
\newcommand{\amone}{\ce{^{241}Am}}
\newcommand{\radon}{\ce{^{222}Rn}}
\newcommand{\thoron}{\ce{^{220}Rn}}
%---
\DeclareSIUnit\c{\mbox{$c$}}
\DeclareSIUnit\year{yr}
\DeclareSIUnit\electron{\mbox{$e^-$}}
\DeclareSIUnit\inch{in}
%---
\newcommand{\adsurl}[1]{\href{#1}{ADS}} 
\providecommand{\url}[1]{\href{#1}{#1}} 
\providecommand{\newblock}{}
%---
\setlength{\unitlength}{1in}
%---
\renewcommand{\thepage}{\arabic{page}}
\newcommand\todo[1]{\textcolor{red}{#1}}

\newcommand{\1}[1]{\, \mathrm{#1}} % unit(y ;-)
\newcommand{\n}[1]{\mathrm{#1}}    % normal (roman) text in math mode
\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{\texttt{arXiv:#1}}}
